One Representation per Word - Does it make Sense for Composition?

In this paper, we investigate whether an a priori disambiguation of word senses is strictly necessary or whether the meaning of a word in context can be disambiguated through composition alone. We evaluate the performance of off-the-shelf single-vector and multi-sense vector models on a benchmark phrase similarity task and a novel task for word-sense discrimination. We find that single-sense vector models perform as well or better than multi-sense vector models despite arguably less clean elementary representations. Our findings furthermore show that simple composition functions such as pointwise addition are able to recover sense specific information from a single-sense vector model remarkably well.

==> _tables/bow_1-4.tex <==
\begin{table*}[!htb]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | c | c | c | c || c | c | c | c || c | c | c | c || c | c | c | c  }
%\hline
\multicolumn{17}{c}{\textbf{Symmetric context window of size 1}}\\
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.53$ & $0.32$ & $0.25$ & $0.14$ & $0.50$ & $0.35$ & $0.15$ & $0.16$ & $0.47$ & $0.32$ & $0.23$ & $0.19$ & $0.47$ & $0.31$ & $0.23$ & $0.18$\\
\textbf{Word Overlap} & $0.63$ & $0.46$ & $0.47$ & $0.40$ & $0.52$ & $0.41$ & $0.31$ & $0.26$ & $0.55$ & $0.40$ & $0.37$ & $0.34$ & $0.54$ & $0.44$ & $0.38$ & $0.29$\\ \hline
\textbf{\texttt{word2vec}} & $\textbf{0.70}$ & $0.56$ & $\textbf{0.61}^{\dagger}$ & $0.54$ & $\textbf{0.59}$ & $0.30$ & $0.54$ & $0.33$ & $\textbf{0.66}^{\ddagger}$ & $\textbf{0.52}$ & $\textbf{0.50}$ & $0.44$ & $\textbf{0.63}^{\dagger}$ & $\textbf{0.56}$ & $\textbf{0.52}$ & $\textbf{0.43}$\\
\textbf{\texttt{dep2vec}} & $0.65$ & $\textbf{0.64}^{\ddagger}$ & $0.57$ & $\textbf{0.57}$ & $0.57$ & $\textbf{0.46}$ & $0.38$ & $0.39$ & $0.64$ & $0.50$ & $0.49$ & $\textbf{0.48}$ & $\textbf{0.63}^{\dagger}$ & $0.55$ & $0.50$ & $\textbf{0.43}$\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $0.67$ & $0.54$ & $0.56$ & $0.56$ & $0.55$ & $0.35$ & $\textbf{0.58}$ & $\textbf{0.44}$ & $0.64$ & $0.49$ & $\textbf{0.50}$ & $0.43$ & $0.62$ & $0.53$ & $0.49$ & $0.38$  \\ \hline\hline
\multicolumn{17}{c}{\textbf{Symmetric context window of size 2}}\\
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.53$ & $0.32$ & $0.25$ & $0.14$ & $0.50$ & $0.35$ & $0.15$ & $0.16$ & $0.47$ & $0.32$ & $0.23$ & $0.19$ & $0.47$ & $0.31$ & $0.23$ & $0.18$\\
\textbf{Word Overlap} & $0.66$ & $0.51$ & $0.55$ & $0.43$ & $0.53$ & $0.43$ & $0.46$ & $0.32$ & $0.59$ & $0.47$ & $0.43$ & $0.41$ & $0.58$ & $0.51$ & $0.45$ & $0.36$\\ \hline
\textbf{\texttt{word2vec}} & $0.70$ & $0.64$ & $0.58$ & $0.55$ & $\textbf{0.62}$ & $0.43$ & $0.62$ & $0.50$ & $\textbf{0.71}^{\ddagger}$ & $\textbf{0.63}^{\ddagger}$ & $\textbf{0.59}^{\ddagger}$ & $0.54$ & $\textbf{0.68}^{\dagger}$ & $0.64$ & $\textbf{0.58}$ & $\textbf{0.49}$\\
\textbf{\texttt{dep2vec}} & $0.71$ & $\textbf{0.65}$ & $0.58$ & $\textbf{0.57}$ & $0.55$ & $0.43$ & $\textbf{0.65}$ & $\textbf{0.56}$ & $0.70$ & $0.57$ & $0.55$ & $\textbf{0.55}$ & $0.66$ & $0.64$ & $0.54$ & $0.46$\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $\textbf{0.72}^{\ddagger}$ & $0.62$ & $\textbf{0.61}$ & $0.52$ & $\textbf{0.62}$ & $\textbf{0.54}$ & $0.58$ & $0.50$ & $0.69$ & $0.56$ & $0.57$ & $0.51$ & $0.67$ & $\textbf{0.65}^{\ddagger}$ & $0.57$ & $0.45$  \\\hline\hline
\multicolumn{17}{c}{\textbf{Symmetric context window of size 4}}\\
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.53$ & $0.32$ & $0.25$ & $0.14$ & $0.50$ & $0.35$ & $0.15$ & $0.16$ & $0.47$ & $0.32$ & $0.23$ & $0.19$ & $0.47$ & $0.31$ & $0.23$ & $0.18$\\
\textbf{Word Overlap} & $0.67$ & $0.55$ & $0.58$ & $0.51$ & $0.57$ & $\textbf{0.41}$ & $0.46$ & $0.32$ & $0.62$ & $0.50$ & $0.49$ & $0.45$ & $0.59$ & $0.55$ & $0.50$ & $0.40$\\ \hline
\textbf{\texttt{word2vec}} & $0.71$ & $0.65$ & $\textbf{0.65}$ & $\textbf{0.57}$ & $\textbf{0.66}$ & $0.38$ & $0.46$ & $0.39$ & $\textbf{0.73}^{\ddagger}$ & $\textbf{0.61}^{\ddagger}$ & $\textbf{0.62}^{\ddagger}$ & $\textbf{0.57}$ & $\textbf{0.71}^{\ddagger}$ & $\textbf{0.62}^{\dagger}$ & $\textbf{0.57}$ & $\textbf{0.53}$\\
\textbf{\texttt{dep2vec}} & $0.72$ & $\textbf{0.66}$ & $0.60$ & $0.54$ & $0.55$ & $\textbf{0.41}$ & $\textbf{0.58}$ & $\textbf{0.44}$ & $0.71$ & $0.55$ & $0.56$ & $0.53$ & $0.67$ & $0.62$ & $0.54$ & $0.50$\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $\textbf{0.75}^{\ddagger}$ & $0.59$ & $0.62$ & $0.55$ & $0.59$ & $0.32$ & $\textbf{0.58}$ & $\textbf{0.44}$ & $0.69$ & $0.57$ & $0.58$ & $0.53$ & $0.68$ & $0.62$ & $0.55$ & $0.47$  \\
\end{tabular}}
\captionsetup{singlelinecheck=false,font=small,labelsep=newline}
\caption{Performance overview for all parts-of-speech and number of senses, $\ddagger$ statistically significant at the $p<0.01$ level; $\dagger$ statistically significant at the $p<0.05$ level}
\label{results_linear_window_all}
\end{table*} 

==> _tables/bow_1.tex <==
\begin{table*}[!htb]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | c | c | c | c || c | c | c | c || c | c | c | c || c | c | c | c | }
%\hline
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c|}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$\\
\textbf{Word Overlap} & $0.62$ & $0.54$ & $\textbf{0.61}$ & $0.55$ & $0.55$ & $0.38$ & $0.54$ & $\textbf{0.44}$ & $0.58$ & $0.48$ & $0.49$ & $0.47$ & $0.58$ & $0.53$ & $0.48$ & $\textbf{0.46}$\\ \hline
\textbf{\texttt{word2vec}} & $\textbf{0.70}^{\dagger}$ & $0.56$ & $\textbf{0.61}$ & $0.54$ & $\textbf{0.59}$ & $0.30$ & $0.54$ & $0.33$ & $\textbf{0.66}^{\ddagger}$ & $\textbf{0.52}$ & $\textbf{0.50}$ & $0.44$ & $\textbf{0.63}^{\dagger}$ & $\textbf{0.56}$ & $\textbf{0.52}$ & $0.43$\\
\textbf{\texttt{dep2vec}} & $0.65$ & $\textbf{0.64}^{\dagger}$ & $0.57$ & $\textbf{0.57}$ & $0.57$ & $\textbf{0.46}$ & $0.38$ & $0.39$ & $0.64$ & $0.50$ & $0.49$ & $\textbf{0.48}$ & $\textbf{0.63}^{\dagger}$ & $0.55$ & $0.50$ & $0.43$\\
%\textbf{PPMI} & & & & & & & & & & & & & & & &\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $0.67$ & $0.54$ & $0.56$ & $0.56$ & $0.55$ & $0.35$ & $\textbf{0.58}$ & $\textbf{0.44}$ & $0.64$ & $0.49$ & $\textbf{0.50}$ & $0.43$ & $0.62$ & $0.53$ & $0.49$ & $0.38$  \\
%\textbf{\APT} & & & & & & & & & & & & & & & & \\
%\textbf{Skip-Thought} & & & & & & & & & & & & & & & & \\ \hline
\end{tabular}}
\captionsetup{singlelinecheck=false,font=small,labelsep=newline}
\caption{LINEAR CONTEXT WINDOW RESULTS, $\dagger$ blabla $\ddagger$ blablbala}
\label{results_linear_window}
\end{table*} 

==> _tables/bow_2.tex <==
\begin{table*}[!htb]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | c | c | c | c || c | c | c | c || c | c | c | c || c | c | c | c | }
%\hline
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c|}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$\\
\textbf{Word Overlap} & $0.63$ & $0.59$ & $0.60$ & $0.54$ & $0.50$ & $0.43$ & $0.62$ & $0.39$ & $0.61$ & $0.52$ & $0.52$ & $0.54$ & $0.63$ & $0.56$ & $0.54$ & $\textbf{0.50}$\\ \hline
\textbf{\texttt{word2vec}} & $0.70$ & $0.64$ & $0.58$ & $0.55$ & $\textbf{0.62}$ & $0.43$ & $0.62$ & $0.50$ & $\textbf{0.71}^{\ddagger}$ & $\textbf{0.63}^{\ddagger}$ & $\textbf{0.59}^{\ddagger}$ & $0.54$ & $\textbf{0.68}^{\dagger}$ & $0.64$ & $\textbf{0.58}$ & $0.49$\\
\textbf{\texttt{dep2vec}} & $0.71$ & $\textbf{0.65}$ & $0.58$ & $\textbf{0.57}$ & $0.55$ & $0.43$ & $\textbf{0.65}$ & $\textbf{0.56}$ & $0.70$ & $0.57$ & $0.55$ & $\textbf{0.55}$ & $0.66$ & $0.64$ & $0.54$ & $0.46$\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $\textbf{0.72}^{\ddagger}$ & $0.62$ & $\textbf{0.61}$ & $0.52$ & $\textbf{0.62}$ & $\textbf{0.54}$ & $0.58$ & $0.50$ & $0.69$ & $0.56$ & $0.57$ & $0.51$ & $0.67$ & $\textbf{0.65}^{\ddagger}$ & $0.57$ & $0.45$  \\
\end{tabular}}
\captionsetup{singlelinecheck=false,font=small,labelsep=newline}
\caption{LINEAR CONTEXT WINDOW 2 RESULTS, $\dagger$ blabla $\ddagger$ blablbala}
\label{results_linear_window}
\end{table*} 

==> _tables/bow_4.tex <==
\begin{table*}[!htb]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | c | c | c | c || c | c | c | c || c | c | c | c || c | c | c | c | }
%\hline
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c|}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$\\
\textbf{Word Overlap} & $0.59$ & $0.61$ & $0.58$ & $\textbf{0.57}$ & $0.53$ & $\textbf{0.46}$ & $\textbf{0.58}$ & $0.33$ & $0.66$ & $0.54$ & $0.55$ & $0.59$ & $0.61$ & $0.58$ & $0.54$ & $\textbf{0.57}$\\ \hline
\textbf{\texttt{word2vec}} & $0.71$ & $0.65$ & $\textbf{0.65}$ & $\textbf{0.57}$ & $\textbf{0.66}$ & $0.38$ & $0.46$ & $0.39$ & $\textbf{0.73}^{\ddagger}$ & $\textbf{0.61}^{\ddagger}$ & $\textbf{0.62}^{\ddagger}$ & $0.57$ & $\textbf{0.71}^{\ddagger}$ & $\textbf{0.62}^{\dagger}$ & $\textbf{0.57}$ & $0.53$\\
\textbf{\texttt{dep2vec}} & $0.72$ & $\textbf{0.66}$ & $0.60$ & $0.54$ & $0.55$ & $0.41$ & $\textbf{0.58}$ & $\textbf{0.44}$ & $0.71$ & $0.55$ & $0.56$ & $0.53$ & $0.67$ & $0.62$ & $0.54$ & $0.50$\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $\textbf{0.75}^{\ddagger}$ & $0.59$ & $0.62$ & $0.55$ & $0.59$ & $0.32$ & $\textbf{0.58}$ & $\textbf{0.44}$ & $0.69$ & $0.57$ & $0.58$ & $0.53$ & $0.68$ & $0.62$ & $0.55$ & $0.47$  \\
\end{tabular}}
\captionsetup{singlelinecheck=false,font=small,labelsep=newline}
\caption{LINEAR CONTEXT WINDOW 4 RESULTS, $\dagger$ blabla $\ddagger$ blablbala}
\label{results_linear_window}
\end{table*} 

==> _tables/dep_1.tex <==
\begin{table*}[!htb]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | c | c | c | c || c | c | c | c || c | c | c | c || c | c | c | c | }
%\hline
& \multicolumn{4}{c||}{\textbf{Adjective}} & \multicolumn{4}{c||}{\textbf{Adverb}} & \multicolumn{4}{c||}{\textbf{Noun}} & \multicolumn{4}{c|}{\textbf{Verb}}\\
\textbf{Senses} & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5 & 2 & 3 & 4 & 5  \\ \hline
\textbf{Random} & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$ & $0.50$ & $0.33$ & $0.25$ & $0.20$\\
\textbf{Word Overlap} & $0.63$ & $0.50$ & $0.55$ & $0.45$ & $0.48$ & $0.43$ & $\textbf{0.38}$ & $0.44$ & $0.61$ & $0.53$ & $0.52$ & $0.48$ & $0.63$ & $0.55$ & $0.52$ & $0.47$\\ \hline
\textbf{\texttt{word2vec}} & $\textbf{0.70}$ & $0.60$ & $0.59$ & $\textbf{0.59}$ & $0.57$ & $0.32$ & $0.27$ & $0.50$ & $\textbf{0.67}$ & $\textbf{0.56}$ & $\textbf{0.59}$ & $\textbf{0.52}$ & $0.65$ & $0.57$ & $\textbf{0.58}$ & $\textbf{0.49}$\\
\textbf{\texttt{dep2vec}} & $0.68$ & $\textbf{0.62}$ & $\textbf{0.61}$ & $0.57$ & $\textbf{0.59}$ & $0.35$ & $0.31$ & $\textbf{0.61}$ & $0.66$ & $0.52$ & $0.54$ & $0.47$ & $0.63$ & $0.55$ & $0.52$ & $0.47$\\
%\textbf{PPMI} & & & & & & & & & & & & & & & &\\
\textbf{{\textsc{Sens}\textsc{Embed}}} & $\textbf{0.70}$ & $0.54$ & $0.55$ & $0.57$ & $0.53$ & $\textbf{0.49}$ & $0.31$ & $0.50$ & $\textbf{0.67}$ & $0.53$ & $0.53$ & $0.51$ & $\textbf{0.70}$ & $\textbf{0.59}$ & $0.57$ & $\textbf{0.49}$  \\
%\textbf{\APT} & & & & & & & & & & & & & & & & \\
%\textbf{Skip-Thought} & & & & & & & & & & & & & & & & \\ \hline
\end{tabular}}
\captionsetup{singlelinecheck=false,font=small,labelsep=newline}
\caption{FIRST ORDER COMPOSITION RESULTS}
\label{results_first_order}
\end{table*} 
